Mitigating Edge Machine Learning Inference Bottlenecks: An Empirical Study on Accelerating Google Edge Models

As the need for edge computing grows, many modern consumer devices now contain edge machine learning (ML) accelerators that can compute a wide range of neural network (NN) models while still fitting within tight resource constraints. We analyze a commercial Edge TPU using 24 Google edge NN models (including CNNs, LSTMs, transducers, and RCNNs), and find that the accelerator suffers from three shortcomings, in terms of computational throughput, energy efficiency, and memory access handling. We comprehensively study the characteristics of each NN layer in all of the Google edge models, and find that these shortcomings arise from the one-size-fits-all approach of the accelerator, as there is a high amount of heterogeneity in key layer characteristics both across different models and across different layers in the same model. We propose a new acceleration framework called Mensa. Mensa incorporates multiple heterogeneous ML edge accelerators (including both on-chip and near-data accelerators), each of which caters to the characteristics of a particular subset of models. At runtime, Mensa schedules each layer to run on the best-suited accelerator, accounting for both efficiency and inter-layer dependencies. As we analyze the Google edge NN models, we discover that all of the layers naturally group into a small number of clusters, which allows us to design an efficient implementation of Mensa for these models with only three specialized accelerators. Averaged across all 24 Google edge models, Mensa improves energy efficiency and throughput by 3.0x and 3.1x over the Edge TPU, and by 2.4x and 4.3x over Eyeriss v2, a state-of-the-art accelerator.

==> sections/abstract.tex <==
% !TEX root=../paper.tex

\begin{abstract}
%\begin{spacing}{\paperlinespacing}

The demands of modern consumer devices are pushing machine learning (ML)
inference to the network edge, with on-device computation.
This has resulted in the design of edge ML accelerators that can compute 
a wide range of neural network (NN) models while still fitting within the tight
resource constraints of edge devices.
We analyze a commercial edge accelerator using
24 Google edge NN models, and find that despite the edge-focused efforts on
designing edge accelerators, they suffer from three shortcomings:
(1)~operating significantly below peak throughput,
(2)~operating significantly below theoretical energy efficiency, and
(3)~inefficiently handling memory accesses.
We comprehensively study the characteristics of each layer in all of the
Google edge models, and find that these shortcomings arise from the
one-size-fits-all approach of edge accelerators, as we find that there is
a high amount of heterogeneity in key layer characteristics both
across different models and across different layers in the same model.

% There has been a significant interest in pushing machine learning (ML) inference computation
% to edge devices. 
% %Given the stringent area and power budget of edge platforms, enabling on-device inference has led to
% %a flurry of proposals for edge accelerators. 
% In this work, we conduct an in-depth analysis of
% inference execution across a wide range of state-of-the-art Google edge models on a state-of-the-art
% edge accelerator. Our analysis shows that the accelerator suffers from three major 
% challenges: (1)~operates significantly (75.6\%) lower than peak
% throughput, (2)~operating far below (62.4\%) than the theoretical energy
% efficiency, and (3)~it's memory system design is neither efficient
% nor effective. 
% %To understand the root cause of accelerator challenges, 
% %We delve deeply into each model
% %and make a key observation 
% Our comprehensive analysis shows that there is a significant variation in terms of layer characteristics
% \emph{across} and \emph{even within} each Google edge model. 
% We find that root cause of accelerator challenges is that
% %is the monolithic architecture of 
% the accelerator's key components (dataflow, computing resources, memory system, and
% NoC) are not designed aware of the heterogeneity in layer
% characteristics.
% %the heterogeneity in layers is root cause of those challenges as the 
% %the accelerator's monolithic architecture is not designed
% %aware of the heterogeneity in layer characteristics, and thus, it fails to achieve the
% %desired energy efficiency, throughput, and area efficiency during
% %executing inference across a wide range of emerging edge
% %models.

To combat this inefficiency, we propose a new framework called \titleShort.
\titleShort incorporates multiple heterogeneous ML accelerators, 
each of which 
%is (1)~much smaller than state-of-the-art edge ML accelerators and
caters to the characteristics of a particular subset of models.
At runtime, \titleShort schedules each layer to run on the best-suited
accelerator, accounting for both efficiency and inter-layer dependencies.
In our analysis of the wide range of Google edge models that we study, 
we find that all of the layers naturally group into a small number of clusters,
allowing \titleShort to operate efficiently even with only a few accelerators.
We design an implementation of \titleShort, consisting of three specialized 
accelerators, for our Google edge models.
% In this work, we propose a framework, called \titleShort, to address the afromentioned challenges. 
% Instead of running the entire model on a monolithic accelerator, \titleShort partition models into multiple categories of layers
% that exhibit similar characteristics, and take advantage of heterogeneity in hardware to design
% multiple accelerators where each is customized for a specific category of layers. 
% Based on our comprehensive layer analysis across our models, we
% design three small accelerator where each is fully customized for a group of layers. 
% %In this work, we propose a  for designing edge acceerators: 
% %instead of running the entire model
% % on a monolithic accelerator, (1)~we partition models into multiple categories of layers
% % that exhibit similar characteristics, and (2)~take advantage of heterogeneity in hardware to design
% % multiple accelerators where each is customized for a specific category of layers. 
% %Our idea is inspired based on a key observation from our analysis:
% %while there is a significant variation in layers characteristics,
% %we can still group layers from different models into a few
% %categories based on their common characteristics. We leverage our observation to design
% % three small hardware accelerators that ... [TODO]
Averaged across all of our edge models, \titleShort improves inference energy 
% (\si{\pico\joule}) 
and throughput 
% (\si{\tera\flop\per\second}) 
by 3.0x and 3.1x, while reducing hardware cost 
% (\si{\milli\meter\squared}) 
and improving area efficiency 
% (\si{\tera\flop\per\milli\meter\squared}) 
by 2.8x and 8.9x, over a state-of-the-art edge ML accelerator. 


 

%\end{spacing}
\end{abstract}

==> sections/methodology-full.tex <==
% !TEX root=../appendix.tex

%\IEEEraisesectionheading{\section{Introduction}}
\section{Methodology}
\label{sec:methodology-full}

\subsection{Models \& Simulation} 
We analyze 24 Google edge NN models, which are used
 as benchmarks for the Edge TPU. These models are used in several
 Google mobile applications/products, such as image classification, object detection,
 semantic segmentation, automatic speech recognition, and image captioning. The models are
 specifically developed for edge devices using TensorFlow Lite~\cite{tensorflow-lite}. All models
 are fully 8-bit quantized (i.e., 32-bit floating point tensor parameters are converted
 into 8-bit fixed-point numbers) using a quantization-aware training approach~\cite{quant-aware-training}.
 The models are then compiled using the Edge TPU compiler~\cite{edge-tpu-compiler},
 which generates custom operations that execute on the Edge TPU.
 
\subsection{Energy and Area Analysis}
We build our energy model based on prior works~\cite{google-pim, tetris, conda}, which sums up the total energy consumed by
the accelerator, DRAM, off-chip and on-chip interconnects, and all on-chip buffers. 
%We use the
% simulator performance counters to drive this model. 
We use CACTI-P 6.5~\cite{CACTI} with a \SI{22}{\nano\meter} process technology
 to estimate on-chip buffer energy. We assume that each 8-bit MAC unit consumes \SI{0.2}{\pico\joule\per\bit}. We model
 the DRAM energy as the energy consumed per bit for LPDDR3, using estimates and models from prior works~\cite{tetris, google-pim}.

 We use analyses from prior works~\cite{eyerissv2, tetris, eyeriss-book}
 to estimate the area complexity
and hardware cost of \titleShort. 
 Given that the PE array and on-chip buffers account for 
97.4\% of the total accelerator area~\cite{eyerissv2,tetris}, 
we use the area of on-chip memory (buffer and register file) and the PE array to 
estimate the area complexity. 
Assuming a \SI{45}{\nano\meter} technology, 
each PE takes \SI{0.01}{\milli\meter\squared} 
based on prior work~\cite{tetris}, and we use CACTI~\cite{CACTI} to analyze
on-chip buffer and register file area.

\subsection{Performance Analysis}
For performance analysis, we use an in-house simulator that models the Edge TPU architecture. The
 simulator models major components of the accelerator including the PE array, memory
 system, on-chip network, and dataflow. We heavily modified the simulator to implement our three proposed accelerators
and the software runtime of \titleShort. 
We develop an analytical cost model to determine the performance of each of our proposed dataflows, and integrate
the dataflow performance numbers into our simulator's performance model. We use CACTI-P 6.5~\cite{CACTI}
to adjust buffer access time latency for each of the on-chip buffers in our proposed accelerators. 
Like prior work~\cite{google-pim, tetris, mondrian, conda}, we use the memory bandwidth available 
inside a 3D-stacked memory chip as the memory bandwidth available to the data-centric accelerators
(which reside in the logic layer of the memory). We 
model a 3D-stacked memory based on
the High-Bandwidth Memory (HBM) standard~\cite{hbm}, and use the bandwidth available in
 the logic layer of HBM (\SI{256}{\giga\byte\per\second}), which is 8x more than the bandwidth available (\SI{32}{\giga\byte\per\second}) to
 the compute-centric accelerator and the baseline edge ML accelerator.
To demonstrate that high bandwidth alone is not enough to solve the
efficiency issues of the baseline accelerator, 
we add a hypothetical configuration to our evaluation (\emph{Base+HB}),
where the baseline accelerator has access to the same 8x internal bandwidth
as logic in the logic layer of HBM.


%We use an in-house simulator to model the accelerator performance.


==> sections/oldintro.tex <==

% !TEX root=../paper.tex

%\IEEEraisesectionheading{\section{Introduction}}
\section{Introduction}  
\label{sec:intro}


Modern consumer devices make widespread use of
machine learning (ML).
The ever-growing quantity and complexity of these devices, combined with 
increasing demand for privacy, connectivity, and real-time responses,
has spurred significant interest in pushing ML inference computation to
the edge (i.e., into these devices, instead of in the cloud)~\cite{edge-facebook, edge-nature,eyerissv2}.
Due to the resource-constrained nature of edge platforms, 
there has been a flurry of proposals on developing specialized
energy-efficient high-performance accelerators for on-device inference
(e.g., Google Edge TPU~\cite{edge-tpu}, NVIDIA Jetson~\cite{jetson}, 
Intel Movidius~\cite{movidius}).
At the same time, neural network (NN) algorithms are evolving rapidly,
which has led to a myriad of popular and emerging NN models
(e.g., CNNs~\cite{image-recognition}, LSTMs~\cite{lstm-google},
GRUs~\cite{gru}, Transducers~\cite{transducer, transducer2},
hybrid models~\cite{lrcn,rcnn-google}), 
with each targeting various applications 
(e.g., face detection~\cite{image-recognition},
speech recognition~\cite{transducer,transducer3, lstm-google}, 
translation~\cite{google-translation}, 
image captioning~\cite{rcnn-google,lrcn}).
The heterogeneity of models used in edge devices, combined with the limited
area and power available in such devices, has resulted in edge ML accelerator
designs that are compatible across a wide variety of NN models.

% Machine learning (ML) has become pervasive in consumer applications. Exponential growth in edge
%  devices combined with an ever increasing demand for privacy, connectivity, and real-time latency
%  has spurred significant interest in pushing ML inference computation to edge devices~\cite{edge-facebook, edge-nature,eyerissv2}. Given
%  the resource-constrained nature of edge platforms, enabling on-device inference has led
%  to a flurry of proposals for specialized hardware accelerators (e.g., Google Edge
%  TPU~\cite{edge-tpu}, NVIDIA Jetson~\cite{jetson}, Intel Movidius~\cite{movidius}) tailored for energy and performance efficient
%  inference execution. At the same time, neural network (NN) architectures and algorithms are evolving at
%  a rapid pace which has led to a myriad of NN models (e.g., CNNs~\cite{image-recognition}, LSTMs~\cite{lstm-google},
%  GRUs~\cite{gru}, Transducers~\cite{transducer, transducer2}, hybrid models~\cite{lrcn,rcnn-google}), each targeting various
%  applications (e.g., face detection~\cite{image-recognition},
%  speech recognition~\cite{transducer,transducer3, lstm-google}, translation~\cite{google-translation}, image captioning~\cite{rcnn-google,lrcn}). 
%  Unlike prior proposals on NN accelerators~\cite{eyeriss,tetris,tangram,e-pur} that mostly targets
%  a specific category of models (e.g., CNNs), heterogeneity of edge models necessitates the need for 
%  designing accelerators that can efficiently execute inference across a wide variety of models. 
%  However, stringent area and power constraint of edge devices, coupled with massive changing rate
%  of model topologies, makes it very challenging to design an edge accelerator that can efficiently execute
%  inference across a wide range of models while achieving high energy efficiency (TFLOPS/j), computational throughput
% (TFLOPS/s) and area efficiency (TFLOPS/\SI{}{\milli\meter\squared}).
% % while satisfying area and power constraints of edge devices.

Unfortunately, the need to cater to so many models in a resource-constrained
environment has made it very challenging for edge ML accelerators to
execute all of these models in a way that simultaneously achieves
high energy efficiency (\si{\tera\flop\per\joule}),
computational throughput (\si{\tera\flop\per\second}), and
area efficiency (\si{\tera\flop\per\milli\meter\squared}).
% In this work, we 
We conduct an in-depth analysis of inference execution
 % across a wide range of state-of-the-art Google edge models
 on a baseline accelerator that is modeled after the Google Edge TPU~\cite{edge-tpu}, 
%  (Section~\ref{sec:motiv}). We analyze 24 models
across 24 state-of-the-art Google edge models spanning four popular NN model types:
%  from four different class of edge models: 
(1)~CNNs, 
(2)~LSTMs~\cite{lstm-google}, 
(3)~Transducers~\cite{transducer, transducer3, transducer4}, and 
(4)~RCNNs~\cite{rcnn-google,lrcn}.
Based on our analysis (Section~\ref{sec:motiv}), we find that the accelerator suffers from
 three major shortcomings. First, the utilization of computing resources are consistently
 low across all models, with the accelerator operating 75.6\% lower on average
 %extremely lower 
%(on average 75.6\%)
 than its peak throughput (\SI{2}{\tera\flop\per\second}). 
For Transducer models, as an example, the accelerator achieves less than 1\% of peak throughput.
% For example, the accelerator achieves
% less than 1\% of the theoretical throughput when executing inference on Transducers. 
Second, despite using specialized logic, the accelerator
 operates 62.4\% below its theoretical peak energy efficiency (\si{\tera\flop\per\joule}) on average.
% far below (62.4\% on average) than the theoretical energy efficiency (TFLOPS/j). Finally, 
Third, the accelerator's memory system is often inefficient.
As an example, while the accelerator's large on-chip storage buffers
(e.g., several megabytes) account for a significant portion of energy consumption
(e.g., 48.1\% static and 36.5\% dynamic energy during CNN inference),
they are often ineffective in reducing off-chip accesses, and cannot accommodate
the model parameters of several larger models.
% In particular, we
%  find that on-chip storage buffers account for a significant portion of both 
%  static and dynamic energy (e.g., 48.1\% inference static energy
%  and 36.5\% of dynamic energy for CNNs) and, despite employing large buffers (e.g., several
%  megabytes), they are not effective in reducing off-chip accesses and fail to accommodate
%  the majority of model parameters.


To understand the root cause of these shortcomings, we dive into a comprehensive 
per-layer analysis of each model, and make two key observations.
First, there is significant variation in terms of
 layer characteristics (e.g., type, shape, \si{\flop\per\byte} ratio, footprint, intra- and inter-layer
 dependencies)
% , computational complexity) 
\emph{across} the models. 
For example, Transducer layers differ drastically (by as much as two orders 
of magnitude) from CNN layers on parameter footprint and \si{\flop\per\byte}.
Second, even \emph{within each model}, there is high variation in terms of 
layer types and shapes 
(e.g., pointwise, depthwise, fully-connected, standard convolution, recurrent).
This leads to variation as large as two orders of magnitude across other
layer characteristics within a single model.
% For example, we find
%  that there is a drastic difference (up to 100x) between Transducers and CNN layer characteristics including
%  parameter footprint, FLOPS per byte ratio, and computational intensity. Even \emph{within each model}, we
%  observe that layers exhibit high variation in terms of layer type and shapes (e.g., pointwise,
%  depthwise, fully-connected, standard convolution, recurrent) which leads to high variation 
% (up to 100x) in layer characteristics across the same model.
% %such as FLOPS per byte ratio, activations/parameters footprint, and MAC
% % intensity. 
We find that the dramatic intra-model heterogeneity is often because unlike
traditional models (e.g., \cite{alex-net,vgg}), these edge models employ
% % in layers \emph{within each model} is mostly because
% recent edge models (unlike traditional models~\cite{alex-net,vgg}) employ 
several techniques (e.g., separable convolutions~\cite{squeezenet,mobilenet})
to reduce the computational complexity and footprint of its layers,
in order to make the model more friendly for resource-constrained edge devices. 
 
% These observations led us to pinpoint the source of accelerator challenges: the accelerator key
%  components, including processing element (PE) array, memory system (on-chip buffers 
% and off-chip memory), dataflow, and NoC, are not designed aware
%  of the heterogeneity in layer characteristics. 
While our analysis uncovers the significant heterogeneity that exists in modern layers,
we find that the key components of edge ML accelerators, including the 
processing element (PE) array,
dataflow,
memory system (on-chip buffers and off-chip memory),
and on-chip network,
are oblivious to this heterogeneity, which leads to the 
three accelerator shortcomings that we observe.
Instead, state-of-the-art edge
 accelerators~\cite{movidius, movidius-arch, jetson, eyeriss, tangram,brainwave} typically take a monolithic design approach, where they
 equip the accelerator with a large PE array, large on-chip buffers, and a fixed
 dataflow (e.g., output stationary). While this approach might work for
 a specific group of layers (e.g., traditional convolutional layers with high compute intensity
 and high data reuse), we find that it fails to achieve the desired energy efficiency, throughput, and
 area efficiency across the diverse state-of-the-art edge models.
 One such example 
% we find that one of the major reasons for the accelerator's
% energy/area inefficiency is memory system as it is not designed aware of layer characteristics.
% % For example, we find that the accelerator's memory system is one of the major reasons for the accelerator's poor
% % energy/area efficiency, as it is not designed aware of variation in 
%  %parameters/activations footprint  and  aritmethic intensity across layers.
is the memory system, where state-of-the-art accelerators employ highly overprovisioned 
on-chip buffers
% , which account for 79.4\% and 52.8\% of the total area and static
%  energy (Section~\ref{sec:eval}), while these buffers fail to
that are unable to
 effectively reduce off-chip parameter traffic and provide
 high bandwidth to PEs, leading to PE underutilization. Another example is the fixed
 dataflow used by the accelerators across all layers.
%  which is one of the root sources of PEs underutilization. we find that due
%  to the dramatic variation in layers characteristics,
% %activation/parameter footprint, operational intensity and inter/intra-layer dependencies,
Thanks to the dramatic variation across different layers,
the fixed dataflow often misses spatial/temporal reuse opportunities across layers.
Our goal is to support edge accelerators that are aware of and can exploit
the variation between layers in edge ML models.

To this end, we propose \titleShort, a general framework for heterogeneous
ML acceleration in edge devices.
The key idea of \titleShort is to incorporate multiple heterogeneous accelerators,
each of which is small and tailored to the characteristics of a particular subset of layers,
and to use a runtime scheduler that assigns each layer to the accelerator that is
best suited to the layer's characteristics and inter-layer dependencies.
As we study the characteristics of different layers in our edge models, 
we observe that the layers naturally group into a small number of clusters.
In each cluster, the layers belonging to that cluster have at least one common
characteristic that differs significantly from the layers in other clusters, and
that strongly influences the optimal hardware design for those layers.
As a result, the number of different accelerators that need to be implemented 
using \titleShort is limited to the number of clusters (five for our Google edge models), 
allowing an implementation of \titleShort to fit within the tight constraints
of edge devices.

% %Our goal in this work is to design an edge accelerator that can run inference efficiently across
% %a wide range of edge models while meeting power and area constraints of edge platforms. Toward this end,
%   We propose a different design approach to tackle the aforementioned challenges.
%   Our idea is inspired based on \emph{a key observation} from our analysis: while there is a significant
%   variation in layers characteristics, we can still group layers from different models into 
%   a few categories based on their common characteristics (Section~\ref{sec:proposal:analysis}). 
%   For example, one category mostly includes depthwise layers that typically exhibit similar characteristics
%  %including
%   (e.g., very low parameter footprint, low MAC intensity). In each category, there exists at least one
%   common characteristic 
% %(e.g., parameter reuse, activation footprint, MAC intensity) 
% that dramaticall differs from other categories. 
%   Leveraging this key observation, our idea is that instead of running the entire model on a monolithic
%   accelerator,  (1)~we partition layers of models into different categories with similar characteristics, and 
%   (2)~take advantage of heterogeneity in hardware to design multiple accelerators where each is
%   fully customized for a specific category of layers. Based on this idea, we propose a framework, 
%   called \titleShort, that supports having multiple heterogeneous small accelerators, each fully tailored
%   for the characteristics of a specific group of layers, and features a scheduler which takes
%   an model and a list of accelerators, and schedules each layer on its own optimized accelerator. 

Informed by the clusters that we identify for all of the layers in
our Google edge models, we design an architectural implementation of \titleShort 
that can efficiently execute the models.
Based on the key characteristics that lead to the formation of each cluster,
we find that our accelerator designs need to center around two characteristics
that have the greatest impact on hardware efficiency.
First, we need separate accelerators for compute-centric clusters and for
data-centric clusters.
Layers in compute-centric clusters make heavy use of their
multiply-accumulators (MACs), have small parameter footprints, and
high parameter reuse, requiring only small on-chip buffers and limited
memory bandwidth.
In contrast, layers in data-centric clusters do not use MACs significantly
compared to their compute-centric counterparts, and have high
memory bandwidth requirements, requiring very different hardware resources
from compute-centric layers.
Second, we need separate accelerators to account for different types of
dataflow across the clusters.
We find that the dataflow of an accelerator depends on the amount of
data reuse that exists, along with whether any inter- and/or intra-layer
dependencies are present, and that the choice of dataflow strongly influences
the entire accelerator design.
Notably, we find that multiple clusters share common reuse and dependency
behavior: our compute-centric layer clusters can efficiently make use
of a single dataflow, and we need only two different types of dataflow
for our data-centric layer clusters.
As a result, we need to implement three accelerators in our framework instance:
(1)~one accelerator, \accelA, tailored for compute-centric layers; and
(2)~two accelerators, \accelB and \accelC, customized for data-centric layers.


% %To implement our idea, we need to answer a key question: how many accelerators do we need to efficiently
% %run inference across all categories? 
% We thoroughly study the implications of each category on the accelerator's architecture
% and our examination reveals two critical insights. First, we find that
% these categories can be further classified into two major groups: (1)~compute-intensive categories
%  which have on average higher MAC intensity, lower parameter footprint, and higher parameter reuse among all categories,
%  and (2)~categories with on average significantly lower MAC intensity, lower parameter reuse and
% higher parameter footprint among all categories. Based on this insight, we find that
% we need to support two types of accelerators: (1)~compute-centric (i.e., an accelerator with high
% compute capability, low bandwidth requirement due to high data reuse), and
% (2)~data-centric (i.e., an accelerator with low compute capability, high bandwidth requirement,
% and close proximity to data). Second, by analyzing reuse opportunities and various data type footprint
% within each category, we find that we need to devise three distinct dataflows to be
% able to efficiently support inference execution across all of these categories. 
% This insight is critical because the dataflow affects the design of several key
% components of the accelerator (e.g. memory system, NoC), and thus, the choice 
% of dataflow can determine the number of accelerators we need. Based on these
% two critical insights, we design an instance of our framework, that includes three
% accelerators: (1)~one compute-centric accelerator (Comp-x) tailored for compute-intensive
% categories, and (2)~two data-centric accelerators (Mem1-x and Mem2-x), customized for data-intensive categories. 

\accelA features a customized dataflow, which is designed based on reuse
and footprint of those layers it executes.
%, aiming to
% to reduce buffer size requirement and
% expose reuse opportunities in both parameters and activations.
 The proposed dataflow enables temporal reduction for output activations and spatial multicasting
 for parameters, leading to a significant reduction of on-chip partial sum traffic. We co-design
 \accelA's memory system with our proposed dataflow. The 
 %small activation and parameter footprint of
 %those layers run on Comp-X as well as 
 reuse opportunities exposed by the dataflow, along with specific characteristics of
 the layers that run on \accelA, enable us to 
 significantly reduce the on-chip buffer size (by 16x) compared to the baseline 
state-of-the-art edge ML accelerator.
    %, which in turn, leads to
 %significant reduction of the Comp-X's energy and area cost.
 \accelA features a 32x32 PE array 
 (\SI{2}{\tera\flop\per\second} peak), whose size is selected
based on the MAC intensity of the layers running on the accelerator. 


%We design Mem1-X and Mem2-X based on the characteristics of those layers they execute.
Both \accelB and \accelC feature customized dataflows based on the
reuse and footprint of the layers that they execute. 
\accelB's dataflow is designed to provide temporal reduction opportunities for
output activation. The dataflow takes advantage of intra-cell dependencies in LSTM layers
to improve parameter reuse across cells, reducing off-chip parameter traffic.
\accelC's dataflow is designed to
expose reuse opportunities in parameters and reduce the size of the parameter buffer size.
We co-design the memory systems of both accelerators with our proposed dataflows.
The layer footprints and reuse opportunities exposed 
by our dataflows enable us to significantly reduce the on-chip buffer sizes (by 32x) for
both accelerators compared to the baseline accelerator. 
To provide high bandwidth and close proximity to data, we leverage 3D-stacked memories to
implement both accelerators. Both \accelB and \accelC feature a much
smaller PE array compared to \accelA, due to the low MAC intensity of the layers: 
the peak throughputs of \accelB and \accelC are \SI{128}{\giga\flop\per\second}
and \SI{512}{\giga\flop\per\second}, respectively.



Our evaluation shows that compared to our monolithic state-of-the-art edge ML accelerator,
    \titleShort reduces total inference energy by 66.0\%,
 improves energy efficiency (\si{\tera\flop\per\joule}) by 3.0x, 
 increases PE array utilization by 28.8x, and increases computational throughput (\si{\tera\flop\per\second}) by 3.1x
(averaged across all 24 Google edge models). 
 We find that \titleShort reduces hardware cost by 2.8x,
 and improves area efficiency (\si{\tera\flop\per\milli\meter\squared}) by 8.9x compared to the
 baseline. 
 %The significant reduction in hardware cost is mostly due to customizing memory
 %systems based on layer characteristics which allow us to dramatically shrink the parameter and
 %activation on-chip buffer sizes for Comp-X, Mem1-X and Mem2-X. 
% Given the rapid evolving rate
% of NN architectures and algorithms, we believe \titleShort becomes even more crucial/useful
% for accelerating future models as it gives us the flexibility to plug-and-play an accelerator 
% in case of a new emerging category of layers. 

%Our result shows that \titleShort reduces total inference energy on average by 66.0\% and
% improves energy efficiency (TFLOPS/\SI{}{\joule}) by 3.0X across all models compared to
% the monolithic baseline accelerator. We find that \titleShort dramatically increases the accelerator 
%utilization across all layers, improving PE array utilization by 28.8x. As a result of 
%improving utilization, \titleShort significantly increases computational throughput (on average by 3.1X) across
% all models (8.1X for LSTMs, 4.9X for Transducers, 1.6X for CNNs, and 2.7X for RCNNs) over
% the monolithic baseline accelerator. We find that \titleShort reduces hardware cost by 2.8X
% and improves area efficiency (TFLOPS/\SI{}{\milli\meter\squared}) by 8.9x compared to baseline
% accelerators. 
 %The significant reduction in hardware cost is mostly due to customizing memory
 %systems based on layer characteristics which allow us to dramatically shrink the parameter and
 %activation on-chip buffer sizes for Comp-X, Mem1-X and Mem2-X. 
% Given the rapid evolving rate
% of NN architectures and algorithms, we believe \titleShort becomes even more crucial/useful
% for accelerating future models as it gives us the flexibility to plug-and-play an accelerator 
% in case of a new emerging category of layers. 


We make the following contributions in this work:

\begin{itemize}[leftmargin=1em,nosep]

\item We conduct the first in-depth analysis of how edge ML accelerators operate
across a wide range of state-of-the-art edge models (provided by Google).
Our analysis reveals three key shortcomings of state-of-the-art accelerators:
(1)~significant PE underutilization,
(2)~poor energy efficiency, and
(3)~an inefficient memory system.

\item We comprehensively analyze the key characteristics of each layer in 
Google's edge models. We make two observations from our analysis:
(1)~layer characteristics vary significantly both \emph{across} models
and across layers \emph{within a single model}, and
(2)~the high layer variation is the root cause of accelerator shortcomings.

\item We propose \titleShort, a new framework for efficient edge ML acceleration.
\titleShort employs a few small, specialized accelerators, and includes a 
runtime scheduler that assigns each layer to one of the accelerators based on
layer characteristics and inter-layer communication.
We find that \titleShort is significantly more efficient than a state-of-the-art
edge ML accelerator for our Google edge models, while using
significantly less area.

% \item We conduct the first in-depth analysis of inference execution across a wide range of Google edge models on a state-of-the-art edge ML accelerator and find that the accelerator suffers from three major architectural challenges: (1)~high underutilization of PEs, (2)~low energy efficiency, and (3)~inefficient memory system.
% 
% \item We perform a comprehensive per-layer analysis of Google edge models and make two key observations: (1)~there is a significant variation in terms of layer characteristics \emph{across} and \emph{within} Google edge models, and (2)~the variation in layers characteristics is the root cause of accelerator's challenges.
% 
% \item We propose a novel approach for designing edge ML accelerators which advocates for breaking the monolithic accelerator model into small customized accelerators ... [TODO]
% 
% \item Our result shows that \titleShort improves inference energy (pj) and throughput (TFLOPS/s) by 3.0X and 3.1X while reducing hardware cost (\SI{}{\milli\meter\squared}) and improving area efficiency (TFLOPS/\SI{}{\milli\meter\squared}) by 2.8X and 8.9X over a state-of-the-art edge ML accelerator. 

 \end{itemize}


